Marketing to Children Through Online Targeted Advertising: Targeting Mechanisms and Legal Aspects

Many researchers and organizations, such as WHO and UNICEF, have raised awareness of the dangers of advertisements targeted at children. While most existing laws only regulate ads on television that may reach children, lawmakers have been working on extending regulations to online advertising and, for example, forbid (e.g., the DSA) or restrict (e.g., the COPPA) advertising based on profiling to children. At first sight, ad platforms such as Google seem to protect children by not allowing advertisers to target their ads to users who are less than 18 years old. However, this paper shows that other targeting features can be exploited to reach children. For example, on YouTube, advertisers can target their ads to users watching a particular video through placement-based targeting, a form of contextual targeting. Hence, advertisers can target children by placing their ads in children-focused videos. Through a series of ad experiments, we show that placement-based targeting is possible on children-focused videos and enables marketing to children. In addition, our ad experiments show that advertisers can use targeting based on profiling (e.g., interest, location, behavior) in combination with placement-based advertising on children-focused videos. We discuss the lawfulness of these two practices concerning DSA and COPPA. Finally, we investigate to which extent real-world advertisers are employing placement-based targeting to reach children with ads on YouTube. We propose a measurement methodology consisting of building a Chrome extension to capture ads and instrument six browser profiles to watch children-focused videos. Our results show that 7% of ads that appear in the children-focused videos we test use placement-based targeting. Hence, targeting children with ads on YouTube is not only hypothetically possible but also occurs in practice...

==> todo.tex <==
%\section{Strange results}
%
%\begin{table}
%  \caption{Overlap of ads between profiles \oana{overlap numbers do not make sense, there is a 100\% overlap between P1 and P6 for float ads when P1 has 0 float ads}}
%  \label{tab:overlap}
%  \footnotesize{
%\begin{tabular}{lccc}
%\hline
%\textbf{Profiles} & \textbf{Overlap} & \textbf{Overlap video ads}& \textbf{Overlap float ads} \\ \hline
%P1\&P2 & 8\% & 8\% & 0\% \\
%P3\&P4 & 3\% & 4\%  & 7,6\%        \\
%P5\&P6 & 7\% & 10\%  & 3\%     \\
%P1\&P3 & 42\% & 29\%  & 100\%        \\
%P1\&P6 & 54\% & 29\%  & 100\%        \\
%P3\&P6 & 14\% & 4\%   &38\%       \\
% \hline
%\end{tabular}
%}
%\end{table}
%
%
%
%\update{We can see that for the profiles that have the same parameters (P1\&P2,P3\&P4,P5\&P6) the overlap is small. When it comes to profiles with different settings (P1\&P3,P3\&P6,P1\&P6) the overlap is concise especially for float ads. The highest overlap is between the P1 and P6, as described P1 is the profile that has no Google profile so google knows nothing about this profile, P6 is the persona that has a Google profile with preferences. This can let us think that the more Google have information about the user, the more the user is targeted by ads, even when it's about children designed videos.   }
%


 \section{Notes -- not to be included in the paper}
  \oana{what was the cookie instrumentation? was it cleaned after each video watched?}
\oana{how much time it took to perform the experiment?}
\oana{finally the videos were not watched at the same time as }

\oana{make a differnce between content on Youtubekids that is overly validated, and all possible contentn dedicated to children }

\update{	- European commission seems to have a hard time to label content for minors ? FTC puts this obligation on the content providers. this seems to be a simple solution for very large online platforms. }

% \oana{update these CCS concepts -- search online for the relevant categories}
 
 %\oana{page limit: 8 pages main content + 2 pages appendix + 2 pages references}
 
 %\oana{we need to clalrify somewhere that we look at ads on Youtube not youtube kids}
 
 \oana{refer in the intro to the study that was saying that kids watch 39 minutes per day youtube videos: https://www.mother.ly/life/youtube-advertising-kids/}
 
 \oana{check: \url{https://www.washingtonpost.com/technology/2020/01/06/youtube-overhauls-advertising-data-collection-kids-content/}
 
 \oana{talk somewhere about the monetization models of kids channels: \url{https://www.uscreen.tv/blog/youtube-kids-content-monetization/}}
 
 \oana{check: \url{https://www.washingtonpost.com/technology/2019/09/02/california-adopted-countrys-first-major-consumer-privacy-law-now-silicon-valley-is-trying-rewrite-it/}} -- californaia Privacy law}: Advertising known as contextual, which is not personalized but assumes certain attributes of most viewers, will still be permitted to run alongside children?s content. YouTube?s parent company, Alphabet, doesn?t disclose detailed financial information on the unit and it was unclear what the financial impact of the changes might be for the company.
 
% \oana{cite: Digital advertising and children Jenny Radesky + Common Sense Study: Young Kids and Youtube how toys, games and ads dominate their viewing -- viewed and coded more than 1600 videos } -- they also coded the ads -- really need to check this
 
 
 \url{https://www.uscreen.tv/blog/youtube-kids-content-monetization/}
 

\url{https://www.youtube.com/watch?v=LuScIN4emyo}


 to cite: 
 YouTube channel owners: Is your content directed to children?: \url{https://www.ftc.gov/business-guidance/blog/2019/11/youtube-channel-owners-your-content-directed-children}
 
Creating for YouTube Kids:  \url{https://static.googleusercontent.com/media/www.youtube.com/en//yt/family/media/pdfs/creating-for-youtube-kids-fieldguide.pdf}
 

 New article 13 that took effect starting 2020 in COPPA
 
more than 8 billion dollars was spend on advertising on children and teens in the us in 2017 (\url{https://www.youtube.com/watch?v=lJyDLN4rkbY})
 
 
 primary concerns with children and advertising: -- Matthew Lapierre -- cite his works
 1. developmentally speaking children are a vulnerable audience -- cannot fight back (legal and moral considerations)
 	- children's immature cognitive and affective skills puts them at disadvantage
			-- children are not capable at understanding the intent behind advertising
			-- children cannot resist advertising
 2. advertising encourages unhealthy eating
 	- majoority of foods advetisied is not the ones they should eat 
	- children respons strongly to child friendly advertising cues  (in a study childrend said the food tested better if the package contain a cartoon character)
 3. advertising creates conflict between children and their caregivers
 	- children ask for products they see advertised and argue with parents about purchaisng them -- this creates stress for parents
 
 issues: 
 	-- advertising has become more subtle -- afiliated marketing
	-- parent monitoring has become more diffucult  -- on tv parents can see what kids watch, but you cannot see this when they look at things on the phoen
	
	

%	
% \update{ Many countries around the world already ban child advertising. In Quebec (Canada), Sweden (1991) and Norway
%advertising to children under the age of 12 is illegal. \oana{I do not understand this, is this only on television? if yes how it is applied in order to know who is watching the TV?}
% In the UK, Greece, Denmark and Belgium advertising to children is restricted.} \oana{what does restricted mean?} \oana{you also need to provide links to all the legislations in all the countries.PROPOSITION DE SUPPRESSION}
%
%
%In the European Union, a social network is considered a public place and therefore the same laws apply. \oana{so what are the laws that apply to the public place?}
%In addition, the European Commission is working on a set or rules to for advertising to children online~\cite{XX}.
% \oana{check these resources to get a better idea what the EC is doing: 
%\url{https://www.politico.eu/article/eu-lawmaker-rule-out-online-ads-target-children/}
%\url{https://ec.europa.eu/info/sites/default/files/5_key_principles_9_june_2022.pdf}
%\url{https://ec.europa.eu/info/sites/default/files/online_marketing_to_children_factsheet_web_en__0.pdf}
%\url{https://ec.europa.eu/info/sites/default/files/executive_summary_impact_marketing_children_en.pdf}
%\url{https://digital-strategy.ec.europa.eu/en/policies/expert-group-safer-internet}
%}



\subsection{Business standards on advertising to children} 
\oana{advertisers are creating these alliances where they set standards for advertising. One such alliance is easa (https://www.easa-alliance.org/issues/children/), but there are others. You need to search and see what self-regulations they propose.}
  
	




